Adaptive Online Replanning with Diffusion Models

Diffusion models have risen as a promising approach to data-driven planning, and have demonstrated impressive robotic control, reinforcement learning, and video planning performance. Given an effective planner, an important question to consider is replanning -- when given plans should be regenerated due to both action execution error and external environment changes. Direct plan execution, without replanning, is problematic as errors from individual actions rapidly accumulate and environments are partially observable and stochastic. Simultaneously, replanning at each timestep incurs a substantial computational cost, and may prevent successful task execution, as different generated plans prevent consistent progress to any particular goal. In this paper, we explore how we may effectively replan with diffusion models. We propose a principled approach to determine when to replan, based on the diffusion model's estimated likelihood of existing generated plans. We further present an approach to replan existing trajectories to ensure that new plans follow the same goal state as the original trajectory, which may efficiently bootstrap off previously generated plans. We illustrate how a combination of our proposed additions significantly improves the performance of diffusion planners leading to 38\% gains over past diffusion planning approaches on Maze2D, and further enables the handling of stochastic and long-horizon robotic control tasks. Videos can be found on the anonymous website: \url{https://vis-www.cs.umass.edu/replandiffuser/}.

==> author1.tex <==
\author{%
  Siyuan Zhou \\
  Hong Kong University of Science and Technology \\
  \And
  Yilun Du \\
  Massachusetts Institute of Technology \\
  \And
  Shun Zhang \\
  MIT-IBM Watson AI Lab \\
  \And
  Mengdi Xu \\
  Carnegie Mellon University \\
  \And
  Yikang Shen \\
  MIT-IBM Watson AI Lab \\
  \And
  Wei Xiao \\
  Massachusetts Institute of Technology \\
  \And
  Dit-Yan Yeung \\
  Hong Kong University of Science and Technology \\
  \And
  Chuang Gan \\
  UMass Amherst and MIT-IBM Watson AI Lab \\
}
